Performance of $b$-Jet Identification in the ATLAS Experiment

The identification of jets containing $b$ hadrons is important for the physics programme of the ATLAS experiment at the Large Hadron Collider. Several algorithms to identify jets containing $b$ hadrons are described, ranging from those based on the reconstruction of an inclusive secondary vertex or the presence of tracks with large impact parameters to combined tagging algorithms making use of multi-variate discriminants. An independent $b$-tagging algorithm based on the reconstruction of muons inside jets as well as the $b$-tagging algorithm used in the online trigger are also presented.The $b$-jet tagging efficiency, the $c$-jet tagging efficiency and the mistag rate for light flavour jets in data have been measured with a number of complementary methods. The calibration results are presented as scale factors defined as the ratio of the efficiency (or mistag rate) in data to that in simulation. In the case of $b$ jets, where more than one calibration method exists, the results from the various analyses have been combined taking into account the statistical correlation as well as the correlation of the sources of systematic uncertainty.

==> paper-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

% Title
\AtlasTitle{Performance of $b$-Jet Identification in the ATLAS Experiment}

% Author - this does not work with revtex (add it after \begin{document})
\author{The ATLAS Collaboration}

% Authors and list of contributors to the analysis
% \AtlasAuthorContributor also adds the name to the author list
% Include package latex/atlascontribute to use this
% Use authblk package if there are multiple authors, which is included by latex/atlascontribute
% \usepackage{authblk}
% \renewcommand\Authands{, } % avoid ``. and'' for last author
% \renewcommand\Affilfont{\itshape\small} % affiliation formatting
% \AtlasAuthorContributor{First AtlasAuthorContributor}{a}{Author's contribution.}
% \AtlasAuthorContributor{Second AtlasAuthorContributor}{b}{Author's contribution.}
% \AtlasAuthorContributor{Third AtlasAuthorContributor}{a}{Author's contribution.}
% \AtlasContributor{Fourth AtlasContributor}{Contribution to the analysis.}
% \author[a]{First Author}
% \author[a]{Second Author}
% \author[b]{Third Author}
% \affil[a]{One Institution}
% \affil[b]{Another Institution}

% If a special author list should be indicated via a link use the following code:
% Include the two lines below if you do not use atlasstyle:
% \usepackage[marginal,hang]{footmisc}
% \setlength{\footnotemargin}{0.5em}
% Use the following lines in all cases:
%  \usepackage{authblk}
%  \author{The ATLAS Collaboration%
%  \thanks{The full author list can be found at:\newline
%   \url{https://atlas.web.cern.ch/Atlas/PUBNOTES/ATL-PHYS-PUB-2014-007/authorlist.pdf}}
% }

% Date: if not given, uses current date
%\date{\today}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{PERF-2012-04}

% CERN preprint number
\PreprintIdNumber{CERN-PH-EP-2015-216}

% ATLAS date - arXiv submission; to be filled in by the Physics Office
% \AtlasDate{\today}

% arXiv identifier
% \arXivId{14XX.YYYY}

% HepData record
% \HepDataRecord{ZZZZZZZZ}

% Submission journal and final reference
\AtlasJournal{JINST}
% \AtlasJournalRef{\PLB 789 (2014) 123}
% \AtlasDOI{}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
The identification of jets containing $b$ hadrons is important for the 
  physics programme of the ATLAS experiment at the Large Hadron Collider.
  Several algorithms to identify jets containing $b$ hadrons are described, 
  ranging from those based on the reconstruction of an inclusive secondary vertex
  or the presence of tracks with large impact parameters to combined tagging algorithms
  making use of multi-variate discriminants.
  An independent $b$-tagging algorithm based on the reconstruction of muons inside jets 
  as well as the $b$-tagging algorithm used in the online trigger are also presented.

  The $b$-jet tagging efficiency, the $c$-jet tagging efficiency and the mistag rate 
  for light flavour jets in data
  have been measured with a number of complementary methods.
  The calibration results are presented as scale factors defined as the ratio 
  of the  efficiency (or mistag rate) in data to that in simulation.
  In the case of $b$ jets, where more than one calibration method exists, the results from the various 
  analyses have been combined taking into account the statistical correlation as
  well as the correlation of the sources of systematic uncertainty.
}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

\AtlasVersion{3.0}
\AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/viewauth/AtlasProtected/BTagPaper2012}

% Comment deadline
% \AtlasCoverCommentsDeadline{DD Month 2014}

\AtlasCoverAnalysisTeam{
  Georges Aad,
  Jean-Fran\c{c}ois Arguin,
  Hannah Arnold,
  Yu Bai,
  Peter Berta,
  Jacobo Blanco,
  V\'eroniqe Boisvert,
  Joseph Boudreau,
  Nicolas Bousson,
  Ingo Burmeister,
  Rob Calkins,
  Lucio Cerrito,
  Dhiman Chakraborty,
  Andrea Coccaro,
  Ian Connelly,
  Ben Cooper,
  Neil Cooper-Smith,
  Markus Cristinziani,
  Dominik Duda,
  Hendrik Esch,
  Andrea Favareto,
  Lorenzo Feligioni,
  Andrea Ferretto Parodi,
  Frank Filthaut (*),
  Sebastian Fleischmann,
  %Ford Gaberson,
  Max Goblirsch-Kolb,
  Tobias Golling,
  Ricardo Goncalo,
  Heather Gray,
  Richard Hawkings,
  Lukas Heinrich,
  %Florian Hirsch,
  David Olivier Jamin,
  Jelena Jovicevic,
  % Christian Jung,
  Michael Kagan,
  Alexandre Khanov,
  Vadim Kostyukhin,
  Agnieszka Leyko,
  Thomas Lohse,
  Gvantsa Mchedlidze,
  John Morris,
  James Mueller (*),
  Martin zur Nedden,
  Priscilla Pani,
  Fabrizio Parodi (*),
  Giacinto Piacquadio,
  Matthew Rose,
  Giuseppe Salamanna,
  Ruth Sandbach,
  Kevin Sapp,
  Timothy Scanlon,
  Carlo Schiavi,
  Dimitri Sidorov,
  Giacomo Snidero,
  Sara Strandberg (*),
  Mossadek Talby,
  %Nancy Tannoury,
  Joshuha Thomas-Wilsker,
  Mark Tibbetts,
  Kirika Uchida,
  Michael Ughetto,
  Laurent Vacavant,
  Marco Vanadia,
  Xiaoxiao Wang,
  Gordon Watts,
  Christian Weiser (*),
  Wouter van den Wollenberg,
  Jie Yu,
  R\'{e}mi Zaidan
}

\AtlasCoverEdBoardMember{Markus Elsing~(chair)}
\AtlasCoverEdBoardMember{Guennadi Borissov}
\AtlasCoverEdBoardMember{Nikolaos Konstantinidis}
\AtlasCoverEdBoardMember{Song-Ming Wang}

\AtlasCoverEgroupEditors{atlas-perf-2012-04-editors@cern.ch}
\AtlasCoverEgroupEdBoard{atlas-perf-2012-04-editorial-board@cern.ch}

